Unveiling the Tricks: Automated Detection of Dark Patterns in Mobile Applications

Mobile apps bring us many conveniences, such as online shopping and communication, but some use malicious designs called dark patterns to trick users into doing things that are not in their best interest. Many works have been done to summarize the taxonomy of these patterns and some have tried to mitigate the problems through various techniques. However, these techniques are either time-consuming, not generalisable or limited to specific patterns. To address these issues, we propose UIGuard, a knowledge-driven system that utilizes computer vision and natural language pattern matching to automatically detect a wide range of dark patterns in mobile UIs. Our system relieves the need for manually creating rules for each new UI/app and covers more types with superior performance. In detail, we integrated existing taxonomies into a consistent one, conducted a characteristic analysis and distilled knowledge from real-world examples and the taxonomy. Our UIGuard consists of two components, Property Extraction and Knowledge-Driven Dark Pattern Checker. We collected the first dark pattern dataset, which contains 4,999 benign UIs and 1,353 malicious UIs of 1,660 instances spanning 1,023 mobile apps. Our system achieves a superior performance in detecting dark patterns (micro averages: 0.82 in precision, 0.77 in recall, 0.79 in F1 score). A user study involving 58 participants further shows that \tool{} significantly increases users' knowledge of dark patterns.

==> changelog.tex <==
1. validity: added micro and macro average performance and better explain the metrics used in Table 4 and Section 8.2. Only report the micro average in the abstract (Page 1, 3, 11)
2. discussed the threat to validity about the dataset, user study, participant recruitment, task segmentation, annotation, evaluation in Section 11 (Page 18)
3. discussed the limitations like practicality in Section 10 (Page 17-18)
4. added the inter-rater agreement results in Section 6.2 (Page 10)
5. added additional study details about the procedure, differences between the full survey and 15-min surveys and the detailed demographic distribution of 15min surveys and the full one. (Page 13-14, 19-20)
6. Added the link to the dataset [8] https://zenodo.org/record/8126443 (Page 3)
7. framed the system to note the risk of misuse by app providers (Page 3, 16)
8. explained the background of Rico and Liu's dataset, and the reason we use it in Section 6.1 (Page 9)
9. moved the related work section from the end of the paper to Section 2 (Page 3-4)
10. removed some duplicated mentions on the related work in the background section (Page 4)
11. subsumed the short research question section into corresponding sections (Page 10, 13)
12. provided more descriptive descriptions for some figures (Page 2, 7, 12, 13)
13. fixed the typos recognised by the reviewers and further proofread the paper
